A Sanity Check for AI-generated Image Detection

With the rapid development of generative models, discerning AI-generated content has evoked increasing attention from both industry and academia. In this paper, we conduct a sanity check on "whether the task of AI-generated image detection has been solved". To start with, we present Chameleon dataset, consisting AIgenerated images that are genuinely challenging for human perception. To quantify the generalization of existing methods, we evaluate 9 off-the-shelf AI-generated image detectors on Chameleon dataset. Upon analysis, almost all models classify AI-generated images as real ones. Later, we propose AIDE (AI-generated Image DEtector with Hybrid Features), which leverages multiple experts to simultaneously extract visual artifacts and noise patterns. Specifically, to capture the high-level semantics, we utilize CLIP to compute the visual embedding. This effectively enables the model to discern AI-generated images based on semantics or contextual information; Secondly, we select the highest frequency patches and the lowest frequency patches in the image, and compute the low-level patchwise features, aiming to detect AI-generated images by low-level artifacts, for example, noise pattern, anti-aliasing, etc. While evaluating on existing benchmarks, for example, AIGCDetectBenchmark and GenImage, AIDE achieves +3.5% and +4.6% improvements to state-of-the-art methods, and on our proposed challenging Chameleon benchmarks, it also achieves the promising results, despite this problem for detecting AI-generated images is far from being solved.

==> Figures/figure_ablation.tex <==
\begin{figure*}[t]
    \vspace{-3mm}
    \centering
    \includegraphics[width=\textwidth]{Figures/figs/ablation.pdf}
    \caption{
        \textbf{Visualization of the effectiveness of PFE and SFE Modules.} The absence of our semantic feature extraction module results in numerous AI-generated images exhibiting pronounced semantic errors that are incorrectly classified as real. Similarly, the second row demonstrates that when the patchwise feature extraction module is omitted, many AI-generated images, despite lacking semantic errors, contain subtle underlying noise that also leads to their misclassification as true.
    }
    \label{fig:ablation}
    \vspace{-3mm}
\end{figure*}



==> Figures/figure_radar.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{Figures/figs/fig_radar.pdf}
    \vspace{-1mm}
    \caption{\textbf{Performance of SOTA method, PatchCraft~\cite{zhong2023rich}, under $\mathcal{B}_1$ (left), $\mathcal{B}_2$ (right), and our \textbf{\texttt{Chameleon}} testset.} The boundary line for Acc = 50\% is marked with a dashed line.}
    \label{fig:radar}
\end{figure}


==> Tables/table_b3.tex <==
\begin{table*}[t]
\centering
\vspace{-3mm}
\caption{\textbf{Comparison on the \textbf{\texttt{Chameleon}}.} Accuracy (\%) of different detectors (rows) in detecting real and fake images of \textbf{\texttt{Chameleon}}. For each training dataset, the first row indicates the \textbf{Acc} evaluated on the \textbf{\texttt{Chameleon}} testset, and the second row gives the {\bf Acc} for ``\textbf{fake image / real image}'' for detailed analysis.
}
\vspace{-2mm}
\resizebox{\hsize}{!}{
\scriptsize 
\renewcommand{\arraystretch}{1.0} 
\setlength\tabcolsep{3pt} 

\begin{tabular}{cccccccccc|c}
\toprule
\textbf{Training Dataset}              & \textbf{CNNSpot} & \textbf{FreDect} & \textbf{Fusing} & \textbf{GramNet} & \textbf{LNP}  & \textbf{UnivFD } & \textbf{DIRE} & \textbf{PatchCraft} & \textbf{NPR} & \textbf{AIDE} \\ \midrule
\multirow{2}{*}{\textbf{ProGAN}}       & 56.94    & 55.62            & 56.98    & \textbf{58.94}      & 57.11      & 57.22       & 58.19    & 53.76  & 57.29       & 58.37          \\
                                       & 0.08/99.67    & 13.72/87.12      & 0.01/99.79    & 4.76/99.66      & 0.09/99.97       & 3.18/97.83    & 3.25/99.48                        & 1.78/92.82  & 2.20/98.70   & 5.04/98.46     \\ \cmidrule(l){2-11} 
\multirow{2}{*}{\textbf{SD v1.4}}      & 60.11    & 56.86            & 57.07    & 60.95      & 55.63     & {55.62}       & 59.71    & 56.32     & 58.13    & \textbf{62.60}          \\
                                       & 8.86/98.63                         & 1.37/98.57       & 0.00/99.96    & 17.65/93.50     & 0.57/97.01      & 74.97/41.09      & 11.86/95.67                       & 3.07/96.35  & 2.43/100.00   & 20.33/94.38     \\ \cmidrule(l){2-11} 
\multirow{2}{*}{\textbf{All GenImage}} & 60.89    & 57.22            & 57.09    & 59.81      & 58.52       & 
{60.42}       & 57.83    & 55.70      & 57.81   & \textbf{65.77}          \\
                                       & 9.86/99.25    & 0.89/99.55       & 0.02/99.98    & 8.23/98.58      & 7.72/96.70       & 85.52/41.56      & 2.09/99.73                        & 1.39/96.52   & 1.68/100.00  & 26.80/95.06      \\ \bottomrule
\end{tabular}

}

\label{table:b3}
\vspace{-2mm}
\end{table*} 
